Conditional Poisson Stochastic Beam Search

Beam search is the default decoding strategy for many sequence generation tasks in NLP. The set of approximate K-best items returned by the algorithm is a useful summary of the distribution for many applications; however, the candidates typically exhibit high overlap and may give a highly biased estimate for expectations under our model. These problems can be addressed by instead using stochastic decoding strategies. In this work, we propose a new method for turning beam search into a stochastic process: Conditional Poisson stochastic beam search. Rather than taking the maximizing set at each iteration, we sample K candidates without replacement according to the conditional Poisson sampling design. We view this as a more natural alternative to Kool et. al. 2019's stochastic beam search (SBS). Furthermore, we show how samples generated under the CPSBS design can be used to build consistent estimators and sample diverse sets from sequence models. In our experiments, we observe CPSBS produces lower variance and more efficient estimators than SBS, even showing improvements in high entropy settings.

==> proofs.tex <==

\section{Conditional Poisson Inclusion Probabilities for Sequence Models}\label{app:cp_inc_probs}
We first provide the derivation of \cref{eq:incl-from-grad}:
\mathcheck{\begin{subequations}\begin{align}
    \picp(i) &\defeq \mathrm{Pr}(i \in Y)\\ 
    &= \sum_Y \Q(Y)\mathbbm{1}\{i\in Y\} \label{eq:1} \\
&= \frac{1}{\Z} \sum_{\substack{|Y| = K, \\ i \in Y}} \ \prod_{j \in Y} w_j \label{eq:2}\\
&= \frac{w_i}{\Z} \sum_{\substack{|Y| = K, \\ i \in Y}} \ \prod_{\substack{j \in Y,\\ i \ne j}} w_j \label{eq:3}\\
&= \frac{w_i}{\Z} \frac{\partial \Z}{\partial w_i} \label{eq:4}
\end{align}\end{subequations}}
\noindent where \cref{eq:1} follows from the definition of inclusion probabilities, i.e., the sum of the probability of all sets containing $i$. We then expand  $\Q(Y)$ to its definition in \cref{eq:cp-distrib} in \cref{eq:2}, subsequently moving terms in \cref{eq:3}. Finally, we use the fact that \mathcheck{$\sum_{\substack{|Y| = K}} \ \prod_{\substack{j \in Y}} w_j$} is our normalization constant $Z$; excluding $w_i$ thus gives us $\frac{\partial \Z}{\partial w_i}$.


We use the following notation for the probability of sampling the sequence of beams $Y_1, \dots, Y_{T}$
\mathcheck{\begin{equation}
    \poisson(Y_1, \dots, Y_{T}) = \Q(Y_1\mid Y_0)\cdots\Q(Y_T\mid Y_{T-1})
\end{equation}}
where we can compute $\Q(Y_{t}\mid Y_{t-1})$ easily via equation \cref{eq:cp-distrib} with normalizing constant \cref{eq:naive}. 
Note that computing $\poisson(Y_T)$ is not as straightforward. We must sum the probability of all sequences of beams $Y_1, \dots, Y_{T-1}$ that can result in $Y_T$ with non-zero probability. The probability of the sequence of beams $Y_1, \dots, Y_T$ under the sampling design $\tilde\poisson$, as defined in \cref{sec:high-var} with respect to a single sequence $\yy$ has the following properties:

\begin{lemma}\label{lem:decomposition}
\mathcheck{\begin{subequations}\begin{align}
    \tildeQ(Y_t \mid Y_{t-1}, \yy) &= \frac{\Q(Y_t \mid Y_{t-1})}{\picp(\yy_t \in Y_t \mid Y_{t-1})}\,\mathbbm{1}\{\yy_{\leq t} \in Y_t\}\\ \tilde\poisson(Y_1, \ldots, Y_\nmax) &= \frac{\poisson(Y_1, \ldots, Y_\nmax)}{\prod_{t=1}^{T} \picp(\yy_{\leq t} \in Y_t \mid Y_{t-1})}\,\mathbbm{1}\{\yy' \in Y_\nmax\}
\end{align}\end{subequations}}

\end{lemma}
\begin{proof}


At any time step $t$, sampling  \mathcheck{$Y_t \sim \tildeQ(\cdot \mid Y_{t-1}, \yy)$} is equivalent to sampling $\propto \Q(\cdot \mid Y_{t-1})\mathbbm{1}\{\yy_{\leq t} \in Y_t\}$, which follows from the definition in \cref{eq:beam_cp_p}. Thus, the distribution $\tildeQ(\cdot \mid Y_{t-1})$ is proportional to $\Q$ up to the normalizing constant \mathcheck{$\sum_{Y_t \subseteq \calB_t, |Y_t|=k} \Q(Y_t \mid Y_{t-1})= \picp(\yy_{\leq t} \in Y_t \mid Y_{t-1})$}.  Calculating the exact inclusion probability \mathcheck{$\picp(\yy_{\leq t} \in Y_t \mid Y_{t-1})$} can be done as shown in \cref{sec:cps}. Under this scheme, clearly \mathcheck{$\tildeQ(Y_t \mid Y_{t-1}, \yy) = \frac{\Q(Y_t \mid Y_{t-1})}{\picp(y_t \in Y_t \mid Y_{t-1})}\,\mathbbm{1}\{\yy_{\leq t} \in Y_t\}$.} The probability of sampling $Y_1, \ldots, Y_\nmax$ according to $\tilde{\poisson}$ then becomes 
{\fontsize{10}{12}\selectfont
\mathcheck{\begin{subequations}\begin{align}
    \tilde{\poisson}(Y_1, \ldots, Y_\nmax)
    &=\frac{\Q(Y_1\mid Y_0)\,\mathbbm{1}\{\yy_{\leq 1} \in Y_1\}}{\picp(\yy_{\leq 1}\in Y_1\mid Y_0)}\cdots \frac{\Q(Y_\nmax\mid Y_{\nmax-1})\,\mathbbm{1}\{\yy_{\leq t} \in Y_t\}}{\picp(\yy_{\leq T}\in Y_{T}\mid Y_{\nmax-1})} \\
    = &\frac{\poisson(Y_1, \ldots, Y_\nmax)}{\prod_{t=1}^{T} \picp(\yy_{\leq t} \in Y_t \mid Y_{t-1})}\,\mathbbm{1}\{\yy \in Y_\nmax\}\label{eq:ptilddef}
\end{align}\end{subequations}}}
\end{proof}




% \begin{equation}\label{eq:inc_prob_rewrite}
%     p(\yy \in \BB_{T}) = \sum_{(Y_0, \ldots, Y_{\nmax-1}) \in \mathrm{supp}(p)} \mathbbm{1}\{\yy_{\nmax-1} \in Y_{\nmax-1}\} p(Y_0, \ldots, Y_{\nmax-1})  p(\yy \in Y_\nmax \mid Y_{\nmax-1})
% \end{equation}


\subsection{A High-Variance Estimator}

The expected value of our estimator in \cref{eq:sad-estimator} is $1/\pipoisson(\yy)$.

Define $c(V, k) = \left|\mathrm{supp}(\tildepoisson)\right|$.
\begin{proof}

\mathcheck{\begin{subequations}\begin{align}
    \E_{Y_1, \ldots, Y_T \sim \tildepoisson}\Bigg[\frac{1}{M\cdot c(\vocab,k)} &\sum_{m=1}^M \frac{1}{\prod_{t=1}^T\Q(Y^{(m)}_t \mid Y^{(m)}_{t-1})}\Bigg]\\
    &=\frac{M}{c(\vocab,k) \cdot M}\E_{Y_1, \ldots, Y_T \sim \tildepoisson}\Bigg[\frac{1}{\poisson(Y_1, \ldots, Y_T)}\Bigg]\\
    &= \frac{1}{c(\vocab,k)}\sum_{Y_1, \ldots, Y_T } \frac{\tildepoisson(Y_1, \dots, Y_T)}{\poisson(Y_1, \ldots, Y_T)} \mathbbm{1}\{\yy \in Y_T\}\\
    &= \frac{1}{c(\vocab,k) } \sum_{Y_1, \ldots, Y_T } \frac{\poisson(Y_1, \dots, Y_T)/\pipoisson(\yy)}{\poisson(Y_1, \ldots, Y_T)} \label{line:a}\\
    &= \frac{1}{c(\vocab,k) }\left|\mathrm{supp}(\tildepoisson)\right| \frac{1}{\pipoisson(\yy )} \\
    &=\frac{1}{\pipoisson(\yy)}
\end{align}\end{subequations}}
where \cref{line:a} follows from \cref{lem:decomposition}.
\end{proof}

Further, the variance of this estimator is


%  
\begin{proof}
\mathcheck{
\begin{subequations}
\begin{align}
    \asvar\Bigg[\hatpipoisson^{-1}(\yy)\Bigg] &= \asvar\Bigg[\frac{1}{M\cdot C(\vocab,k)} \sum_{m=1}^M \frac{1}{\prod_{t=1}^T\Q(Y^{(m)}_t \mid Y^{(m)}_{t-1})} \Bigg] \\
     &= \frac{1}{M\cdot c(\vocab,k)^2} \asvar\Bigg[ \frac{1}{\prod_{t=1}^T\Q(Y_t \mid Y_{t-1})}\Bigg] \\
     &= \frac{1}{M\cdot c(\vocab,k)^2} \frac{\mathbb{V}\Bigg[ \prod_{t=1}^T\Q(Y_t \mid Y_{t-1})\Bigg]}{\displaystyle\E_{Y_1, \ldots,Y_T \sim \tildepoisson}\Big[\prod_{t=1}^T\Q(Y_t \mid Y_{t-1})\Big]^4} &\text{\color{gray}(apply the Delta method)}\\
     &= \frac{1}{M\cdot c(\vocab,k)^2} \frac{\mathbb{V}\Big[ \poisson(Y_1, \dots, Y_T)\Big]}{\displaystyle\E_{Y_1, \ldots, Y_T \sim \tildepoisson}\Big[\poisson(Y_1, \ldots, Y_T)\Big]^4} & \text{\color{gray}(substitute definition)} \label{eq:highvar}
    %  \\
    %  &= \frac{1}{M^2\cdot C(\vocab,k)^2} \frac{\E_{Y_0, \dots,Y_T \sim \tilde\poisson}\Big[ \poisson(Y_0, \dots, Y_T)^2\Big] -\E_{Y_0, \dots,Y_T \sim \tilde\poisson}\Big[ \poisson(Y_0, \dots, Y_T)\Big]^2 }{\displaystyle\E_{Y_0, \dots,Y_T \sim \tilde\poisson}\Big[\poisson(Y_0, \dots, Y_T)\Big]^4}
\end{align}
\end{subequations}}
\end{proof}
Moreover, we note that $\mathbb{V}\Big[ \poisson(Y_1, \dots, Y_T) \leq 1$.
this gives us an upper-bound on the variance
\begin{equation}
   \asvar\Bigg[\hatpipoisson^{-1}(\yy)\Bigg]  \leq  \frac{1}{M\cdot c(\vocab,k)^2} \frac{\mathbb{V}\Big[ \poisson(Y_1, \dots, Y_T)\Big]}{\displaystyle\E_{Y_1, \ldots, Y_T \sim \tildepoisson}\Big[\poisson(Y_1, \ldots, Y_T)\Big]^4} 
\end{equation}
A back-of-the-envelopment calculation reveals the following---if we plug in the uniform distribution for $\poisson$, i.e. every possible sequence $Y_1, \ldots, Y_T$, we have that each sequence has probability $\frac{1}{c(V, k)}$, we arrive at
\begin{equation}
   \asvar\Bigg[\hatpipoisson^{-1}(\yy)\Bigg]  \leq  \frac{c(V, k)^2}{M}
\end{equation}
which hints at why the variance is so large in practice. 

While perhaps not immediately obvious, this variance can be extremely high under certain distributions. For example, when $\displaystyle\E_{Y_1, \dots, Y_T \sim \tilde\poisson}\Big[\poisson(Y_1, \dots, Y_T)\Big ]$ is on the order of $\frac{1}{C(\vocab,k)}$, which we may reasonably expect since CPS is a high entropy sampling scheme, then our variance becomes approximately $ \frac{C(\vocab,k)^2}{M}\,\mathbb{V}\Big[ \poisson(Y_1, \dots, Y_T)\Big]$. Even when $\mathbb{V}\Big[ \poisson(Y_1, \dots, Y_T)\Big]$ is low, multiplication by such a large number may cause the variance of our estimator to explode. 
%uniform distribution over all series of sets $Y_0, \dots, Y_T$, i.e., for any  $Y_0, \dots, Y_T$, we have $\Poisson(Y_0, \dots, Y_T) = \frac{1}{M\cdotC(\vocab,k)}$. Under this setting, the denominator in \cref{eq:highvar} becomes $\frac{1}{(M\cdot C(\vocab,k))^4}$. After incorporating the multiplicative constant, the denominator of \cref{eq:highvar} then becomes $\frac{1}{(M\cdot C(\vocab,k))^2}$, i.e.,

% \begin{align}
%     \E_{Y_0, \dots, Y_T \sim\tilde\poisson}[\frac{1}{M\cdot C(\vocab,k)} &\sum_{m=1}^M \frac{1}{\prod_{t=1}^T\Q(Y^{(m)}_t \mid Y^{(m)}_{t-1})}]\\
%     &=\frac{M}{C(\vocab,k) \cdot M}\E_{Y_0, \dots, Y_T \sim \tilde\poisson}[\frac{1}{\poisson(Y_0, \dots, Y_T)}]\\
%     &= \frac{1}{C(\vocab,k)}\sum_{Y_0, \dots, Y_T } \frac{\tilde \poisson(Y_0, \dots, Y_T)}{\poisson(Y_0, \dots, Y_T)} \mathbbm{1}\{\yy \in Y_T\}\\
%     &= \frac{1}{C(\vocab,k) } \sum_{Y_0, \dots, Y_T } \frac{\poisson(Y_0, \dots, Y_T)/\pipoisson(\yy \in  Y_\nmax)}{\poisson(Y_0, \dots, Y_T)} \label{line:a}\\
%     &= \frac{1}{C(\vocab,k) }|\mathrm{supp}(\tilde\poisson)| \frac{1}{\pipoisson(\yy \in  Y_\nmax)} \\
% &=\frac{1}{\pipoisson(\yy \in  Y_\nmax)}
% \end{align}
% where \cref{line:a} follows from \cref{lem:decomposition}.



\subsection{A Monte Carlo estimator for $\pipoisson$}\label{app:mc_proof}
The \defn{asymptotic variance} of the reciprocal of our estimator $\pipoisson^{\textsc{mc}}(\yy)$ defined in \cref{eq:mc-naive} is
\mathcheck{\begin{equation}
\asvar\Big[\left(\pipoisson^{\textsc{mc}}(\yy)\right)^{-1}\Big] = \frac{1}{M}\left(1/\pipoisson(\yy)^3- \frac{1}{\pipoisson(\yy)^2}\right) \nonumber
\end{equation}}


\begin{proof}
As \cref{eq:mc-naive} is a Monte Carlo estimator, it is asymptotically normal and its limiting distribution is \mathcheck{$\calN(\pipoisson(\yy), \sfrac{1}{M})$.}
We seek the limiting distribution of \mathcheck{$g(x) = \sfrac{1}{x}$.
Note $g'(x) = -\sfrac{1}{x^2}$.} 
By the delta method \cite{doob1935}, we have that the limiting distribution of \mathcheck{$g(\pipoisson^{\textsc{mc}}(\yy))$ is $\calN\left(\pipoisson(\yy)^{-1},  g'(\pipoisson(\yy))^2/M \right) = \calN\left(\pipoisson(\yy)^{-1},  1/M\pipoisson(\yy)^4\right)$.}
\end{proof}

The quantity in the denominator, $\pipoisson(\yy)^4$, is typically quite small for large $\calB$ with dispersed weights, which makes the estimator $\pipoisson^{\textsc{mc}}(\yy)$ all but unusable in the context of sequence models.

\subsection{A Better, Consistent Estimator}

%First, note that exact inclusion probabilities can be written as the sum of the probability of all (sequences of) beams such that $\yy$ is in the last beam:
Our estimator $\hat{\pi}^{\textsc{IS}}_{\poisson}(\yy)$\ryan{Needs to be macroed}, defined in \cref{eq:is-good}, 
is an unbiased estimator of $\pipoisson(\yy)$. 
Further, the estimator of the inverse inclusion probabilities $\hat{\pi}^{\textsc{IS}}_{\poisson}(\yy)^{-1}$\ryan{needs to be macroed} is consistent.
%and has asymptotic variance $\asvar\Big[           \hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy)\Big] = \frac{1}{M}$
% Importantly, as the following theorem states, we can take
% the reciprocal and maintain the low variance.

% \begin{theorem} 

% The following estimator of the inverse inclusion probabilities:
% \begin{equation}
% \frac{1}{M}\sum_{m=1}^M \frac{1}{\prod_{t=1}^T \picp(\yy_{\leq t} \in Y_t^{(m)} \mid Y_{t-1}^{(m)})}
% \end{equation}
% is consistent and has asymptotic variance
% \begin{equation}
% \asvar\Big[           \hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy)\Big] = \frac{1}{M}
% \end{equation}
% \end{theorem}
% \begin{equation}
%     p(\yy \in \BB_\nmax) = \sum_{(Y_0, \ldots, Y_\nmax) \in \mathrm{supp}(p)} p(Y_0, \ldots, Y_\nmax) \mathbbm{1}\{\yy \in Y_\nmax\}
% \end{equation}
% Importance sampling estimator
% \begin{align}
%     p(\yy \in \BB_\nmax) &= \sum_{(Y_0, \ldots, Y_\nmax) \in \mathrm{supp}(\tilde{p})} \tilde{p}(Y_0, \ldots, Y_\nmax)\frac{p(Y_0, \ldots, Y_\nmax)}{\tilde{p}(Y_0, \ldots, Y_\nmax)} \mathbbm{1}\{\yy \in Y_\nmax\} \\ 
%     &= \sum_{(Y_0, \ldots, Y_\nmax) \in \mathrm{supp}(\tilde{p})} \tilde{p}(Y_0, \ldots, Y_\nmax)\frac{p(Y_0, \ldots, Y_\nmax)\,\inc(\yy \in Y_\nmax)}{p(Y_0, \ldots, Y_\nmax)} \mathbbm{1}\{\yy \in Y_\nmax\} \\
%       &= \sum_{(Y_0, \ldots, Y_\nmax) \in \mathrm{supp}(\tilde{p})} \tilde{p}(Y_0, \ldots, Y_\nmax)\,p(\yy \in Y_\nmax) \mathbbm{1}\{\yy \in Y_\nmax\} \\
%       &= \sum_{(Y_0, \ldots, Y_\nmax) \in \mathrm{supp}(\tilde{p})} \tilde{p}(Y_0, \ldots, Y_\nmax)\,p(\yy \in Y_\nmax) 
% \end{align}

\begin{proof}
\mathcheck{\begin{subequations}\begin{align}
\E_{Y_T \sim \tildepoisson}\Bigg[\frac{1}{M}\sum_{m=1}^M & \prod_{t=1}^T \picp(\yy_{\leq t} \in  Y_t^{(m)} \mid Y_{t-1}^{(m)}) \Bigg]\\
&= \sum_{Y_T  } \tildepoisson(Y_1, \ldots, Y_\nmax) \prod_{t=1}^{T} \piQ(\yy_{\leq t} \in Y_t \mid Y_{t-1})\\
%&= \sum_{Y_T  } \tildepoisson(Y_1, \ldots, Y_\nmax) \prod_{t=1}^{T} \piQ(\yy_{\leq t} \in Y_t \mid Y_{t-1})  \mathbbm{1}\{\yy \in Y_T\}\\
&= \sum_{Y_T  } \tildepoisson(Y_1, \ldots, Y_\nmax) \frac{\poisson(Y_1, \ldots, Y_\nmax)}{\poisson(Y_1, \ldots, Y_\nmax)} \prod_{t=1}^{T}  \piQ(\yy_{\leq t} \in Y_t \mid Y_{t-1})  \\
&= \sum_{Y_T  } \poisson(Y_1, \ldots, Y_\nmax) \frac{\tildepoisson(Y_1, \ldots, Y_\nmax)}{\tildepoisson(Y_1, \ldots, Y_\nmax)} \mathbbm{1}\{\yy \in Y_T\} \quad \text{\color{gray} {\small insert definition from \cref{eq:ptilddef}}} \\ 
& = \sum_{Y_T  } \poisson(Y_1, \ldots, Y_\nmax)\,\mathbbm{1}\{\yy \in Y_\nmax\} \\ &= \pipoisson(\yy)
\end{align}\end{subequations}}

By the strong law of large numbers, we know that $\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy)$ converges almost surely to $\pipoisson(\yy)$, it's expected value. Recall that the continuous mapping theorem states that 
\mathcheck{\begin{equation}
    X_n \overset{\mathrm{a.s.}}{\rightarrow} X \longrightarrow g(X_n) \overset{\mathrm{a.s.}}{\rightarrow} g(X)
\end{equation}}
for function $g$ with discontinuity points $D_g$ such that $P(X \in D_g) = 0$. Given the function $g(x) = 1/x$, we see that $P(\pipoisson(\yy) = 0 ) = 0$ since all sequences with non-zero weight have some chance of being in the final set under the CPSBS scheme. As such, we can conclude

\mathcheck{\begin{equation}
    \frac{1}{(\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy))} \overset{\mathrm{a.s.}}{\rightarrow} \frac{1}{\pipoisson(\yy)}
\end{equation}}
which means the estimator is consistent. 
\end{proof}
% To show that $(\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy))^{-1}$ is consistent, we need only show that 
% \begin{equation}
%     \lim_{M \rightarrow \infty} P(|\frac{1}{M}\sum_{m=1}^M \prod_{t=1}^T \picp(\yy_{\leq t} \in Y_t^{(m)} \mid Y_{t-1}^{(m)} - \frac{1}{\pipoisson(\yy)}| \geq \epsilon) = 0
% \end{equation}
% \end{proof}
% \begin{proof}
% We use the Delta method to show the asymptotic normality of the estimator $(\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy'))^{-1}$ and subsequently derive its variance. We use the notation $(\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy'))_n$ to indicate that $n$ samples were used in our estimate. 


\inLongVersion{

Proof of variance of the estimator $\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy)$:
\begin{proof}
\begin{align}
\asvar\Big[ &\hat{\pi}^{\mathrm{IS}}_{\poisson}(\yy)\Big]   = \left(\sum_{Y_T \in \mathrm{supp}(\tilde{\poisson})} \poisson(Y_1, \ldots, Y_\nmax)\,\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t^{(m)} \mid Y_{t-1}^{(m)})\right) -\pipoisson(\yy \in Y_T)^2 \\
&= \left(\sum_{Y_T \in \mathrm{supp}(\tilde{\poisson})} \poisson(Y_1, \ldots, Y_\nmax)\,\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t \mid Y_{t-1})\right) - \sum_{Y_T \in \mathrm{supp}(\tilde{\poisson})} \poisson(Y_1, \ldots, Y_\nmax) \pipoisson(\yy \in Y_T) \\
&= \left(\sum_{Y_T \in \mathrm{supp}(\tilde{\poisson})} \poisson(Y_1, \ldots, Y_\nmax)\,\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t \mid Y_{t-1}) - \pipoisson(\yy \in Y_T) \right) \\
&\leq \sum_{Y_T \in \mathrm{supp}(\tilde{\poisson})} \poisson(Y_1, \ldots, Y_\nmax)\,\left|\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t \mid Y_{t-1}) - \pipoisson(\yy \in Y_T) \right| \\
&\leq \sum_{Y_T \in \mathrm{supp}(\tilde{\poisson})} \tilde\poisson(Y_1, \ldots, Y_\nmax)\,\left|\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t \mid Y_{t-1}) - \pipoisson(\yy \in Y_T) \right| \\
&= \E_{Y_T \in \mathrm{supp}(\tilde{\poisson})}\left[\left|\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t \mid Y_{t-1}) - \pipoisson(\yy \in Y_T) \right|\right] \\
     %&\sum_{Y_T\in \mathrm{supp}(\poisson)} \frac{\mathbbm{1}\{\yy \in Y_T\}^2\,\poisson(Y_1, \ldots, Y_\nmax)^2}{\tilde{\poisson}(Y_1, \ldots, Y_\nmax)} \\
     %&=  \sum_{Y_T\in \mathrm{supp}(\poisson)} \frac{\mathbbm{1}\{\yy \in Y_T\}^2\,\poisson(Y_1, \ldots, Y_\nmax)^2\,\pipoisson(\yy \in Y_T)}{\poisson(Y_1, \ldots, Y_\nmax)} \\
     %&=  \sum_{Y_T \in \mathrm{supp}(\poisson)} \mathbbm{1}\{\yy \in Y_T\}^2\,\poisson(Y_1, \ldots, Y_\nmax)\,\prod_{t=1}^T\picp(\yy_{\leq t} \in Y_t^{(m)} \mid Y_{t-1}^{(m)}) \\
   %\pipoisson(\yy \in Y_T)\\
%     &= \pipoisson(\yy \in Y_T)^2 \\
   %  &=  \inc(\yy)^2
\end{align}
\end{proof}}

